Novice programmers strategies for online resource use and their impact on source code

Websites are frequently used by programmers to support the development process. This paper investigates programmer-Web interactions when coding, and combines observations of behaviour with assessments of the resulting source code. We report on an online observational study with ten undergraduate student programmers as they engaged in programming tasks of varying complexity. Screens were recorded of participants' activities, and each participated in an interview. Videos and interviews were thematically analysed. Novice programmers employed various strategies for seeking and utilising online knowledge. The resulting source code was examined to determine the extent to which it met requirements and whether it contained errors. The source code analysis revealed that coding with the websites involved more coding time and effort, but increased the possibility of producing correct code. However, coding with websites also introduced instances of either incorrect or non-executable source code.

==> Unused/02a_resources.tex <==
% \section{Coding resources}

% ADDING CHASE PAPERS.

% Add if needed:
    % Data workers further consider the use of external resources, including Google and \SO{} to strengthen their coding while using established codebases, as \citet{hanUnderstandingDataWorker2020} found in a lab-based experiment.

% Developers make substantial use of the web when programming \cite{acar2016you, brandt2009two, michaels2020empirical, xia2017}. Search engines, for example, are used for activities such as program comprehension and code reuse \cite{hora2021, maalejComprehensionProgramComprehension2014, xia2017}, debugging \cite{hora2021, xia2017}, and background knowledge acquisition and reference (including \eg{} syntax) \cite{hora2021, xia2017}. The \StackOverflow{} Q\&A website has been observed to dominate programming-related online search \cite{acar2016you, hora2021, xia2017} and is often used in preference to official documentation \cite{ragkhitwetsagulToxicCodeSnippets2019} -- for example, in their observation study of $60$ industry developers, \cite{xia2017} find that 63\% of all searches involve a visit to the website \cite{xia2017}. In analysing programmers search queries, \cite{hora2021} found found that Google were used to search and referred to \StackOverflow{} (11\%), YouTube (6\%), and W3school (5\%) websites. \cite{brandt2009two} investigate how the programmers use the websites during development by observing 20 students while coding and manually analysing 300 search query sessions. They found that programmers use websites for learning aid by locating tutorial websites and for clarifications by searching unknowing terms even when debugging. In a study of Jupyter notebook, \cite{koenzenCodeDuplicationReuse2020} study a sample of 500 duplicate code extracted from GitHub then check for duplicate in Jupyter notebooks, and perform an observational study with 8 graduate students form CS and chemistry. Participants were asked to solve three tasks with varying difficulties. They audio recorded participants discussion and recorded their screens. They found that online were the most used resources for coding, and online searching accumulate of 18\% of participants’ time, involve searching for repetitive task even if it was searched recently. Tutorials were most visited websites, followed by API documentation and \StackOverflow. 
% In this paper, we examine developers usage of the resources, with a particular focus on the web. Our observations provide a rich understanding about the role of the web within in-practice coding, and how other resources supplement such usage. 
 
 


==> Unused/02c_methods.tex <==
\subsection{Method for recording and analysing videos} 
% Caroline notes:
    % "it's sort of more people have tried to automate this, but methods aren't reliable". Not related to the discussion about using the online resources. Again, say " Here I am manually coding the video, because automated methods don't work reference kind of thing. ". Aim is justify.
    % Do not include details about the automated: not your method. Justify your method.

The study used participants' video recordings to observe behaviours during coding sessions and employed a manual way to code the videos. Different methods have been proposed to record programmers' behaviours using logged data. For example, recording browser and online searching activities \cite{astromskisPatternsDevelopersBehaviour2017, sadowski2015developers, liuCharacterizingSearchActivities2021}, and IDE events \cite{schroerRecordingVisualisingUnderstanding2021, fuchsMonitoringStudentsMobile2014}. Adopting logged data are suitable to capture the activities. However, such methods make it difficult to capture detailed information about behaviours and interpret the data definitively. An alternative way is using the qualitative observation method to capture behaviours and interactions  \cite{seamanQualitativeMethodsEmpirical1999}. Such a method capture observations of the phenomena to gain a deep understanding with high realism without manipulating variables or settings \cite{stol2018abc}. Video recordings could be used to observe behaviours, which decrease human errors and bias, ensure iterative exposure to the events, allow multiple aspects of the captured behaviour, and perform with inexpensive cost \cite{seamanQualitativeMethodsEmpirical1999, bakeman2012behavioral}. Screen recordings comprises of videos that ensure capturing details information of the ongoing activities \cite{robillardHowEffectiveDevelopers2004, koExploratoryStudyHow2006, fuchsMonitoringStudentsMobile2014, baiExploringToolsStrategies2019}, which proved to reduce the Hawthorne effect \cite{shaochunxuDialogbasedProtocolEmpirical2005}. 

It was argued that observing software development is limited because much of the work on the developer's head, where logging low-level data, such as keystrokes and mouse events, is a substitute approach \cite{seamanQualitativeMethodsEmpirical1999}. Nevertheless, many details about the coding processes were undiscovered, especially when using the websites. In another matter, it was claimed that coding the video files using automated tools facilitates such a process \cite{baoExtractingAnalyzingTimeseries2017, baoInferenceDevelopmentActivities2018}. While these tools save time and effort, extracting fine-grained details from coding the videos is still challenging, and human interventions are still required. The manual video coding still requires more time and effort but ensures a more robust way to generate rich data, and it is not prone to missing some behaviours.
 
 
 
% For more Info:
    % -What are the setting of the observations? See https://www.scribbr.com/methodology/observational-study/
    % Why recording behaviours is important? What results could be benefiting? This mean also why using the observation? Rich data maybe and exploring. 
    % (Astromskis et al., 2017): has a really interesting LR about the visual and tools both used to observe behaviours. 
    % One point to add in regards of Gaps: the current papers are either focus on education, or miss the qualitative ways by watching the videos.
% suggested section from the introduction:
    %     LR: method-log files- needs LR section from Ch5. 
    %     areas-debugging 


%  From Old Introduction: study of behaviours and gap 
    %     Programmer is an essential part of coding who engage various resources to collect and process information, and help in writing and compiling the code. We know anecdotally that using websites while programming is an essential part of programming. Thus, examining the underpinning process that led to producing the output is an area that received attention with an aim to enhance the programmers' experience. Prior work investigate the log files produced by the programmers. \cite{bliksteinUsingLearningAnalytics2011} in his paper studied the logs file of students to infer their behaviours during coding. Also, other research focused mainly on specific areas of the coding like debugging \cite{meierBehaviourPatternsLearners2020}, and the produced errors while compiling \cite{jadudFirstLookNovice2005}. Further, the time spent by programmers and the possible interruptions received an interest \cite{parninResumptionStrategiesInterrupted2011}. While these studies provide interesting observations of the programmers' behaviours, addressing the programmers' behaviours in light of the used resources that presumably takes space in the programming sessions to unveil their employed strategies is not yet explored. 

% --------------OLD LR-----------------------------------------

% \subsection{Using log files}

% There are many papers in the filed where they performed various metrics and tools to assess participants behaviours mainly novice; metrics that are related to the students and novice performance include Error Quotient that mainly concerns the encountered of syntax errors (Jadud 2006), Watwin Score as an improvement of the EQ (Watson et al., 2013), and NPSM that include semantic not only the syntax (Carter et al. 2015), and RED (Bret Becker). While these metrics provide enormous benefit on predicting and enhancing novice performance, it focuses only on one part of the programming session and how novice produce and tackle syntax and semantic errors. Our focus is much more broad covering all the possible programmers behaviours observed during programming session with the use of websites. 

% Different tools have used to collect and analyse programming information. Log files were the most dominated type of data given it accessible way of recording and automatically analyse the data. There are ready to use tools such as NetLogo (Blikstein, 2011), "Test My Code" plugin in NetBeans IDE (Vihavainen et al, 2014), BlueJ (Jadud, 2005); other developed their own tools such as Blackbox data set that collect users’ data based on BlueJ plugin (Brown et al, 2014), a web-based tool to record students’ programming activity (Helminen et al.,2013), and a "PROM" to record log file including the browser history (Astromskis et al., 2017), and (Jadud).
% Recoding the data using qualitative approach is also conducted. Screen recording the programmers activities to extract the used strategies is conducted without any focused on the actually video and the source code (Ko et al, 2006). An attempt to make the process faster by developing and using an automatic video analysis tools called: scvRipper which provide in-depth granularity of the data that exceed the need; yet, it missed some required elements (Bao et. al, 2015). Using qualitative method provide endless amount of information to analyse which in one side is time-consuming but in other side reveal fruitful details help uncover the actual behaviours; yet, there are still a scarce in the use of qualitative method in collecting and analysing the programmer behaviours.


% /////////////////////////////////////////////
% Data
% (Blikstein, 2011) tutorial to fetch the code, copy and paste
% The observed behaviors and the narrative are based on tools that record the compilations and code size, but missed what actually occurred on the coding.  Using NetLogo’s log file, the paper did analysis 9 programmers files assessing their compilation events, the number of characters (increase the code size), time using unscripted task to infer and predict any possible patterns 

% (Carter et al. 2015): proposed and derived NPSM to measure students performance and compared it explanatory power against EQ and WS
% It might worth plotting about the EQ, WS and NPSM as all predict students performance? (Is it related?)

% (Vihavainen et al, 2014) NetBeans IDE plugin “My code” to record subject snapshots.

% (Estacio and Raga Jr, 2017): Using log files from various course that used Moodle learning environments

% (Brown et al, 2014) This paper is based on the “Blackbox” data set that collect users’ data based on BlueJ blugin

% (Helminen et al.,2013) In-brwoser Python environment include: editor, executive environment, and an interactive Python console: to record students’ programming activity.

% (Astromskis et al., 2017): similar intention but different method: Record programmers logs using PROM tool; their own tool that collect interaction with events, time, and the contents. Their tool called PROM which collected Logs not videos, and then classified based on the contents of each log.

% (Jadud, 2005) & EQ paper for Jadud: BlueJ of novice compilation. 

% % //Videos:
% (Ko et al, 2006) Screen recording the programmers

% (Bao et. al, 2015) scvRipper: (using automatic video analysis): provide in-depth trangility of the data that exceed the need, and missed some required elements. 


% Notes: more papers are toward making findings to the pedagogical field. 

% \subsection{Focusing on specific area}
% Studying programmers behaviours is a vast area that encamps many parts where many papers have address them. For example, addressing the processes around the debugging process and its outcome (Murphy et al., 2008), the errors made and its relation with performance (Jadud, 2005), the quality of the produced code (Astromskis et al., 2017), the link between the exhibited behaviours and success (Robillard et al., 2004), the behaviours pattern (Meier et al., 2020), information quest (Ko et al, 2006), time spent navigation (Astromskis et al., 2017), and interruption and resumption (Parnin and Rugaber, 2011). 

% Our intention is to record the observed behaviours while coding using the websites, and qualitatively analyse these behaviours to produce rich understanding about the actual behaviours, which then help to infer what kind of strategies that differ the normal programming flow causing more time and effort, and effect the produce code. The strategies is similar to (Ko et al, 2006, Meier et al., 2020) but our strategies is more related to the online resources. Also, we analyse the produce source code similar to  (Astromskis et al., 2017) but we used systematic tools rather than a previous method that work well for long code snippets. 


% OUR INTENTION IS NOT PEDGAGOCIAL, YET WE ARE INTESRESTED TO OBSERVE possible impact from the use of external resources on the programming processes and the output. 

% MISSING:
% Data:
% Writing the first code: (Vihavainen et al, 2014)
% General: (Fuchs et al. 2014)
% (Astromskis et al., 2017): time, navigation, SRC quality
% (Ko et al, 2006): Seek, Relate, and Collect Relevant Information during Software Maintenance Tasks
% (Meier et al., 2020):behaviour patterns of different learners in solving programming tasks
% (Robillard et al., 2004): Explore the behaviors exhibited while investigating code and it links with the success of such process. Following a methodical is more beneficial than opportunities.

% (Parnin and Rugaber, 2011): Interruption and resumption
